Perception of emergent epidemic of COVID-2019 / SARS CoV-2 on the Polish Internet

We study the perception of COVID-2019 epidemic in Polish society using quantitative analysis of its digital footprints on the Internet (on Twitter, Google, YouTube, Wikipedia and electronic media represented by Event Registry) from January 2020 to 12.03.2020 (before and after official introduction to Poland on 04.03.2020). To this end we utilize data mining, social network analysis, natural language processing techniques. Each examined internet platform was analyzed for representativeness and composition of the target group. We identified three temporal major cluster of the interest before disease introduction on the topic COVID-2019: China- and Italy-related peaks on all platforms, as well as a peak on social media related to the recent special law on combating COVID-2019. Besides, there was a peak in interest on the day of officially confirmed introduction as well as an exponential increase of interest when the Polish government declared war against disease with a massive mitigation program. From sociolingistic perspective, we found that concepts and issues of threat, fear and prevention prevailed before introduction. After introduction, practical concepts about disease and epidemic dominate. We have found out that Twitter reflected the structural division of the Polish political sphere. We were able to identify clear communities of governing party, mainstream oppostition and protestant group and potential sources of misinformation. We have also detected bluring boundaries between comminities after disease introduction.

==> img_dir/table2.tex <==
\begin{table}[ht]
\centering
\begin{tabular}{llll}
\toprule
kolejnosc & item & count & percent\\
\midrule
1 & Dziś & 447 & 0.0179\\
2 & 14 & 421 & 0.0169\\
3 & Minister & 401 & 0.0161\\
4 & Głosowanie & 291 & 0.0117\\
5 & Premier & 283 & 0.0113\\
\addlinespace
6 & Rząd & 199 & 0.0080\\
7 & Prezydent & 187 & 0.0075\\
8 & Panie & 182 & 0.0073\\
9 & Epidemia & 180 & 0.0072\\
10 & Donald & 178 & 0.0071\\
\addlinespace
11 & Objawy & 163 & 0.0065\\
12 & Polska & 148 & 0.0059\\
13 & .@M\_K\_Blonska & 143 & 0.0057\\
14 & Sławomir & 140 & 0.0056\\
15 & Lekarze & 131 & 0.0053\\
\addlinespace
16 & Podstawowe & 129 & 0.0052\\
17 & Szef & 126 & 0.0051\\
18 & Mamy & 122 & 0.0049\\
19 & Wygadywanie & 118 & 0.0047\\
20 & .@StKarczewski & 116 & 0.0047\\
\addlinespace
21 & Świat & 114 & 0.0046\\
22 & Pierwszy & 110 & 0.0044\\
23 & Niestety & 105 & 0.0042\\
24 & Propozycja & 102 & 0.0041\\
25 & Wszyscy & 102 & 0.0041\\
\addlinespace
26 & Zakończyło & 100 & 0.0040\\
27 & Przewodniczący & 95 & 0.0038\\
28 & INFORMACJA & 92 & 0.0037\\
29 & Odnoszę & 89 & 0.0036\\
30 & Wczoraj & 85 & 0.0034\\
\addlinespace
31 & Pacjent & 81 & 0.0032\\
32 & Kolejne & 78 & 0.0031\\
33 & Włochy & 74 & 0.0030\\
34 & Strach & 65 & 0.0026\\
\bottomrule
\end{tabular}
\end{table}


==> img_dir/table21.tex <==
\begin{adjustbox}{width=\columnwidth,center}
\begin{tabular}{ cc }
  \centering
% top level tables, with 2 rows
% bottom left of the top level table: table 1
\begin{tabular}{clll}
\toprule
Id & item & count & item en\\
\midrule
1 & Dziś & 447 & today\\
2 & 14 & 421 & 14\\
3 & Minister & 401 &Minister\\
4 & Głosowanie & 291 & Voting\\
5 & Premier & 283 & Prime Minister\\
6 & Rząd & 199 & Government\\
7 & Prezydent & 187 & President\\
8 & Panie & 182 & Mr\\
9 & Epidemia & 180 & Epidemic\\
10 & Donald & 178 & Donald\\
11 & Objawy & 163 & Symptoms\\
12 & Polska & 148 & Poland\\
13 & .@M\_K\_Blonska & 143 & candidate_pres\\
14 & Sławomir & 140 & Sławomir\\
15 & Lekarze & 131 & Physicians\\
16 & Podstawowe & 129 & Basics\\
17 & Szef & 126 & Chef\\
\bottomrule
\end{tabular} &
% starting bottom right of the top level table
% table 2
\begin{tabular}{clll}
\toprule
id & item & count & item_en\\
\midrule
18 & Mamy & 122 &we have\\
19 & Wygadywanie & 118 & talking\\
20 & .@StKarczewski & 116 & v-ce pres_Senat)\\
21 & Świat & 114 &World\\
22 & Pierwszy & 110 &First\\
23 & Niestety & 105 &unfortunately\\
24 & Propozycja & 102 & proposition\\
25 & Wszyscy & 102 & All\\
26 & Zakończyło & 100 & Finished\\
27 & Przewodniczący & 95 & Chairman\\
28 & INFORMACJA & 92 &information\\
29 & Odnoszę & 89 &Answering\\
30 & Wczoraj & 85 & Yesterday\\
31 & Pacjent & 81 & Patient\\
32 & Kolejne & 78 & next\\
33 & Włochy & 74 & Italy\\
34 & Strach & 65 & fear\\
\bottomrule
\end{tabular}\\
\end{tabular}
\end{adjustbox}


==> img_dir/table2_-_Copy.tex <==
\begin{adjustbox}{width=\columnwidth,center}
\begin{tabular}{ cc }
  \centering
% top level tables, with 2 rows
% bottom left of the top level table: table 1
\begin{tabular}{clll}
\toprule
kolejnosc & item & count & percent\\
\midrule
1 & Dziś & 447 & 0.0179\\
2 & 14 & 421 & 0.0169\\
3 & Minister & 401 & 0.0161\\
4 & Głosowanie & 291 & 0.0117\\
5 & Premier & 283 & 0.0113\\
6 & Rząd & 199 & 0.0080\\
7 & Prezydent & 187 & 0.0075\\
8 & Panie & 182 & 0.0073\\
9 & Epidemia & 180 & 0.0072\\
10 & Donald & 178 & 0.0071\\
11 & Objawy & 163 & 0.0065\\
12 & Polska & 148 & 0.0059\\
13 & .@M\_K\_Blonska & 143 & 0.0057\\
14 & Sławomir & 140 & 0.0056\\
15 & Lekarze & 131 & 0.0053\\
16 & Podstawowe & 129 & 0.0052\\
17 & Szef & 126 & 0.0051\\
\bottomrule
\end{tabular} &
% starting bottom right of the top level table
% table 2
\begin{tabular}{clll}
\toprule
kolejnosc & item & count & percent\\
\midrule
18 & Mamy & 122 & 0.0049\\
19 & Wygadywanie & 118 & 0.0047\\
20 & .@StKarczewski & 116 & 0.0047\\
21 & Świat & 114 & 0.0046\\
22 & Pierwszy & 110 & 0.0044\\
23 & Niestety & 105 & 0.0042\\
24 & Propozycja & 102 & 0.0041\\
25 & Wszyscy & 102 & 0.0041\\
26 & Zakończyło & 100 & 0.0040\\
27 & Przewodniczący & 95 & 0.0038\\
28 & INFORMACJA & 92 & 0.0037\\
29 & Odnoszę & 89 & 0.0036\\
30 & Wczoraj & 85 & 0.0034\\
31 & Pacjent & 81 & 0.0032\\
32 & Kolejne & 78 & 0.0031\\
33 & Włochy & 74 & 0.0030\\
34 & Strach & 65 & 0.0026\\
\bottomrule
\end{tabular}\\
\end{tabular}
\end{adjustbox}


==> img_dir/table3.tex <==
\begin{table}[ht]
\centering
\begin{tabular}{clr}
\toprule
kolejnosc & konto & centralosc\\
\midrule
1 & MichalSzczerba & 949\\
2 & Leszczyna & 914\\
3 & MZ\_GOV\_PL & 820\\
4 & PremierRP & 800\\
5 & Platforma\_org & 654\\
\addlinespace
6 & AndrzejTurczyn & 590\\
7 & KONFEDERACJA\_ & 538\\
8 & MiroslawSuchon & 520\\
9 & KrzysztofBrejza & 494\\
10 & idzpodpradpl & 468\\
\addlinespace
11 & M\_K\_Blonska & 443\\
12 & GIS\_gov & 406\\
13 & MikiWrobelek\_ & 360\\
14 & prezydentpl & 356\\
15 & Bart\_Wielinski & 344\\
\addlinespace
16 & AndrzejDuda & 331\\
17 & LewitujacyUmysl & 326\\
18 & Jowita\_W & 298\\
19 & PiotrMuller & 283\\
20 & KChojecka & 280\\
\addlinespace
21 & michalrachon & 274\\
22 & KancelariaSejmu & 269\\
23 & PawelChojecki & 263\\
24 & pigmalion55 & 263\\
25 & KosiniakKamysz & 234\\
\addlinespace
26 & ADReverse & 205\\
\bottomrule
\end{tabular}
\end{table}



==> img_dir/table31.tex <==
\begin{adjustbox}{width=\columnwidth,center}
\begin{tabular}{ cc }
  \centering
\begin{tabular}{clr}
\toprule
item & account & centrality\\
\midrule
1 & MichalSzczerba & 949\\
2 & Leszczyna & 914\\
3 & MZ\_GOV\_PL & 820\\
4 & PremierRP & 800\\
5 & Platforma\_org & 654\\
6 & AndrzejTurczyn & 590\\
7 & KONFEDERACJA\_ & 538\\
8 & MiroslawSuchon & 520\\
9 & KrzysztofBrejza & 494\\
10 & idzpodpradpl & 468\\
11 & M\_K\_Blonska & 443\\
12 & GIS\_gov & 406\\
13 & MikiWrobelek\_ & 360\\
\bottomrule
\end{tabular} &
\begin{tabular}{clr}
\toprule
item & account & centrality\\
\midrule
14 & prezydentpl & 356\\
15 & Bart\_Wielinski & 344\\
16 & AndrzejDuda & 331\\
17 & LewitujacyUmysl & 326\\
18 & Jowita\_W & 298\\
19 & PiotrMuller & 283\\
20 & KChojecka & 280\\
21 & michalrachon & 274\\
22 & KancelariaSejmu & 269\\
23 & PawelChojecki & 263\\
24 & pigmalion55 & 263\\
25 & KosiniakKamysz & 234\\
26 & ADReverse & 205\\
\bottomrule
\end{tabular}\\
\end{tabular}
\end{adjustbox}


==> img_dir/table3_-_Copy.tex <==
\begin{adjustbox}{width=\columnwidth,center}
\begin{tabular}{ cc }
  \centering
\begin{tabular}{clr}
\toprule
kolejnosc & konto & centralosc\\
\midrule
1 & MichalSzczerba & 949\\
2 & Leszczyna & 914\\
3 & MZ\_GOV\_PL & 820\\
4 & PremierRP & 800\\
5 & Platforma\_org & 654\\
6 & AndrzejTurczyn & 590\\
7 & KONFEDERACJA\_ & 538\\
8 & MiroslawSuchon & 520\\
9 & KrzysztofBrejza & 494\\
10 & idzpodpradpl & 468\\
11 & M\_K\_Blonska & 443\\
12 & GIS\_gov & 406\\
13 & MikiWrobelek\_ & 360\\
\bottomrule
\end{tabular} &
\begin{tabular}{clr}
\toprule
kolejnosc & konto & centralosc\\
\midrule
14 & prezydentpl & 356\\
15 & Bart\_Wielinski & 344\\
16 & AndrzejDuda & 331\\
17 & LewitujacyUmysl & 326\\
18 & Jowita\_W & 298\\
19 & PiotrMuller & 283\\
20 & KChojecka & 280\\
21 & michalrachon & 274\\
22 & KancelariaSejmu & 269\\
23 & PawelChojecki & 263\\
24 & pigmalion55 & 263\\
25 & KosiniakKamysz & 234\\
26 & ADReverse & 205\\
\bottomrule
\end{tabular}\\
\end{tabular}
\end{adjustbox}

